Robust Tracking via Mamba-based Context-aware Token Learning

How to make a good trade-off between performance and computational cost is crucial for a tracker. However, current famous methods typically focus on complicated and time-consuming learning that combining temporal and appearance information by input more and more images (or features). Consequently, these methods not only increase the model's computational source and learning burden but also introduce much useless and potentially interfering information. To alleviate the above issues, we propose a simple yet robust tracker that separates temporal information learning from appearance modeling and extracts temporal relations from a set of representative tokens rather than several images (or features). Specifically, we introduce one track token for each frame to collect the target's appearance information in the backbone. Then, we design a mamba-based Temporal Module for track tokens to be aware of context by interacting with other track tokens within a sliding window. This module consists of a mamba layer with autoregressive characteristic and a cross-attention layer with strong global perception ability, ensuring sufficient interaction for track tokens to perceive the appearance changes and movement trends of the target. Finally, track tokens serve as a guidance to adjust the appearance feature for the final prediction in the head. Experiments show our method is effective and achieves competitive performance on multiple benchmarks at a real-time speed. Code and trained models will be available at https://github.com/GXNU-ZhongLab/TemTrack.

==> figs/fig-attn.tex <==
\begin{figure}[t] %双栏的图带星号
    \centering
    \includegraphics[width=8.4cm,height=6cm]{CameraReady/LaTeX/attn.pdf}%width=\linewidth height=6.4cm
    \caption{
    Visualize the attention of search to {\mytoken}.
    The first column is ground truth, the second column is the attention in the last layer of the backbone, and the third column is the attention in {\mymodule}.
    }
    \label{fig-attn}
\end{figure}

==> figs/fig-box.tex <==
\begin{figure}[t] %双栏的图带星号
    \centering
    \includegraphics[width=8.4cm,height=3.5cm]{CameraReady/LaTeX/vis_bbox.pdf}
    \caption{
    Comparison tracking results with the other three SOTA trackers on LaSOT\cite{lasot} benchmark.
    }
    \label{fig-box}
\end{figure}

==> figs/fig-zhizhuwang.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=8.4cm]{CameraReady/LaTeX/eao.pdf}
    \caption{AUC scores of difference attributes on LaSOT\cite{lasot}. Best viewed in color.}
    \label{fig:zhizhuwang}
\end{figure} 
 


==> figs/fig1.tex <==
\begin{figure}[t] %双栏的图带星号
    \centering
    \includegraphics[width=7.6cm,height=4.8cm]{CameraReady/LaTeX/scatter_plot.png}%width=\linewidth height=6.4cm
    \caption{
    Comparison of different types of trackers.
    (a) The common trackers focus on appearance modeling.
    (b) Current SOTA trackers combine temporal information extraction and appearance modeling by inputting more images (or features).
    (c) Our tracker models appearance and learns temporal information separately, extracting temporal information between representative {\mytoken}s.
    }
    \label{fig1}
\end{figure}

==> figs/fig2.tex <==
% 框架图
\begin{figure*}[t] %双栏的图带星号
    \centering
    \includegraphics[width=17.5cm]{CameraReady/LaTeX/fig2.pdf}%width=\linewidth height=6.4cm
    \caption{
    Overview of the proposed tracker {\mytracker}. 
    The tracker's workflow is depicted from left to right, including feature extraction \& interaction, temporal information modeling, and the final head stage.
    First, we add a {\mytoken} $f_t$ concatenating with template and search tokens to gather the target's appearance in the backbone.
    Furthermore, we develop {\mymodule} to associate {\mytoken}s to dig temporal information.
    Finally, the {\mytoken} guides the adjustment of the search feature to achieve more accurate predictions in the head network.
    }
    \label{fig2}
\end{figure*}

==> figs/fig3.tex <==
\begin{figure}[t] %双栏的图带星号
    \centering
    \includegraphics[width=8cm, height=7cm]{CameraReady/LaTeX/fig3.pdf}%width=\linewidth height=6.4cm
    \caption{The schematic diagram of the Mamba\_Cross. The $f_t$ and $H_t$ indicate {\mytoken} and the hidden state at the $t$ frame, respectively. In this module, the {\mytoken} $f_t$ gathers the appearance of the previous frames within a sliding window.}
    \label{fig3}
\end{figure}

==> figs/quxiantu.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=8.4cm,height=4.3cm]{CameraReady/LaTeX/quxiantu.pdf}
    \caption{Success plots of one-pass evaluation (OPE) about fast motion and full occlusion challenges on LaSOT.
    Best viewed in color and zooming in.
    }
    \label{fig:quxian}
\end{figure} 
 


==> tables/tab-ablation.tex <==
% \begin{table}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \fontsize{9}{12}\selectfont
%     \begin{tabular}{cc|ccc}
%     \toprule
%       &  AUC & P$_{norm}$ & P\\
%      \midrule
%      Baseline &  &  & \\
%      +{\mytoken} &  &  & \\ %不进行时序建模，直接指导search
%      +{\mymodule} &  &  & \\
%     \bottomrule 
%     \end{tabular}
%         }
        
%     \caption{ Ablation study for important components. Blank denotes the component is used by default, while \ding{55} represents the component is removed. Performance is evaluated on LaSOT\cite{lasot}.}
    
%     \label{tab:ablation}
% \end{table} 


\begin{table*}[ht]
\centering
    \begin{minipage}{0.3\linewidth}
    %     \centering
    %     % \resizebox{\linewidth}{!}{
    %     \fontsize{9}{9}\selectfont
    %     \begin{tabular}{c|cc|cc}
    %     \toprule 
    %      \multirow{2}{*}{Method}  &\multicolumn{2}{c|}{LaSOT} &\multicolumn{2}{c}{GOT10K}  \\
    %      & AUC & P$_{norm}$ & AO & SR$_0.5$ \\
    %      \midrule
    %      Baseline  & \bred{71.2}  & 81.2 & 78.2\\
    %      +{\mytoken} &  &  & \\ %不进行时序建模，直接指导search
    %      +{\mymodule} & 72.0 & 82.1 & 79.1 \\
    %     \bottomrule 
    %     \end{tabular}
    %     % }
    % \caption{Ablation studies of {\mytracker}.}
    % \label{tab:ablation}
    \centering
        % \resizebox{\linewidth}{!}{
        \fontsize{9}{10}\selectfont
        \begin{tabular}{c|c|ccc}
        \toprule
         m & n & AUC & P$_{norm}$  & P \\
         \midrule
         2  & 16 & 71.1 & 81.2 & 78.2\\
         4  & 8  & 71.9 & 82.0 & 79.0\\
         8  & 4  & 72.0  & 82.1 & 79.1\\
         % 16 & 2  &  & & \\
        \bottomrule 
        \end{tabular}
        % }    
    \caption{Influence of the window size.}
    \label{tab:temporal_number}
    \end{minipage}
    % \hfill
    \hspace{0.02\textwidth}
    \begin{minipage}{0.29\linewidth}
        \centering
        % \resizebox{\linewidth}{!}{
        \fontsize{9}{7}\selectfont
        \begin{tabular}{c|c|ccc}
        \toprule
         Backbone & Our\_method  & AUC \\% & P$_{norm}$ & P\\
         \midrule
         % ViT        &  &  & \\
         \multirow{2}{*}{HiViT} & - & \bred{69.4} \\% & 80.7 & 77.3\\ %不进行时序建模，直接指导search
         & \checkmark & 70.5\\
         \midrule
         \multirow{2}{*}{Fast-iTPN}  & -  & 71.1 \\%& 82.1 & 79.1\\
         & \checkmark & 72.0 \\
        \bottomrule 
        \end{tabular}
        % }
    \caption{Influence of the backbone.}
    \label{tab:backbone}
    \end{minipage}
    % \hfill
    \hspace{0.01\textwidth} % Space between the tables
    \begin{minipage}{0.3\linewidth}
        \centering
        % \resizebox{\linewidth}{!}{
        \fontsize{9}{10}\selectfont
        \begin{tabular}{c|ccc}
        \toprule
         Component     &  AO & SR$_{0.5}$ \\%&SR$_{0.75}$ \\%& P\\
         \midrule
         % \textbf{Mamba\_Cross}   & \textbf{72.5(+1.3)} & \textbf{82.9} \\% & \textbf{80.1} \\
         % Self\_Cross           & 71.8(+0.6) & 82.0 \\%& 78.9\\ %不进行时序建模，直接指导search
         % Self\_Self            & 72.0(+0.8) & 82.2 \\%& 79.4 \\
         Mamba\_Cross          & 74.9 & 84.8 \\%& 71.7 \\% & \textbf{80.1} \\
         Self\_Cross           & 74.3 & 84.6 \\%& 71.7\\%& 78.9\\ %不进行时序建模，直接指导search
         Self\_Self            & 74.2 & 84.2 \\%& 70.8 \\%& 79.4 \\
         % Cross + Mamba  & & & \\
        \bottomrule 
        \end{tabular}
        % }
    \caption{Influence of different layers.}
    \label{tab:temporal_module}
    \end{minipage}
    % \caption{Ablation studies and different components of the {\mytracker}-256 on LaSOT\cite{lasot}.}
    \label{tab:mytrack}
\end{table*}

==> tables/tab1.tex <==
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{
%     \fontsize{8}{9}\selectfont
%     \begin{tabular}{r|c|ccc|ccc|ccc|cc|c}
%     \toprule
%     \multicolumn{1}{c|}{\multirow{2}{*}{Method} }
%     & \multicolumn{1}{c|}{\multirow{2}{*}{Source}} 
%     & \multicolumn{3}{c|}{LaSOT} 
%     & \multicolumn{3}{c|}{LaSOT$_{ext}$} 
%     & \multicolumn{3}{c|}{GOT-10K$^*$} 
%     & \multicolumn{2}{c|}{TNL2K}
%     & \multicolumn{1}{c}{UAV123}\\ 
%     \cline{3-14}
%                                             && AUC & $\rm P_{norm}$ & P     & AUC & $\rm P_{norm}$ & P      & AO & $\rm SR_{0.5}$ & $\rm SR_{0.75}$     & AUC & P & AUC \\
%     \midrule
%     \textbf{{\mytracker}-256} & Ours                 & \bred{72.0} & \bred{82.1} & \bred{79.1}      &\bred{52.4} & \bred{63.3} & \bred{60.2} & \bred{74.9} & \bred{84.8} & 71.7  &\bblu{58.8} & \bred{60.9} &\bred{70.8}\\
%     \midrule
%     AQATrack-256\cite{AQATrack} & CVPR24    & 71.4 & \bblu{81.9} & \bblu{78.6}    & \bblu{51.2} & \bblu{62.2} & \bblu{58.9}    & 73.8 & 83.2 & \bred{72.1}    & 57.8 & \bblu{59.4} & \bblu{70.7}\\
%     % ARTrackv2-256\cite{artrackv2} & CVPR24  & \bblu{71.6} & 80.2 & 77.2    & 50.8 & 61.9 & 57.7    & 75.9 & 85.4 & 72.7    & \bred{59.2} & -    & 69.9\\
%     EVPTrack-224\cite{evptrack} &AAAI24     & 70.4 & 80.9 & 77.2    & 48.7 & 59.5 & 55.1    & 73.3 & 83.6 & 70.7    & \bblu{59.1} & 57.5 & 70.2 \\
%     F-BDMTrack-256\cite{F-BDMTrack}&ICCV23  & 69.9 & 79.4 & 75.8    & 47.9 & 57.9 & 54.0    & 72.7 & 82.0 & 69.9    & 56.4 & 56.5 & 69.0 \\
%     ROMTrack-256\cite{ROMTrack} & ICCV23    & 69.3 & 78.8 & 75.6    & 48.9 & 59.3 & 55.0    & 72.9 & 82.9 & 70.2    & -    & -    & 69.7 \\
%     ARTrack-256\cite{ARTrack} & CVPR23      & 70.4 & 79.5 & 76.6    & 46.4 & 56.5 & 52.3    & 73.5 & 82.2 & 70.9    & 57.5 & -    & 67.7 \\
%     SeqTrack-B256\cite{seqtrack} & CVPR23   & 69.9 & 79.7 & 76.3    & 49.5 & 60.8 & 56.3    & \bblu{74.7} & \bblu{84.7} & \bblu{71.8}    & 54.9 & -    & 69.2 \\
%     VideoTrack\cite{VideoTrack1}  & CVPR23  & 70.2 & - & 76.4       & -    & -    & -       & 72.9 & 81.9 & 69.8    & -    & -    & 69.7 \\
%     MixFormer-22k\cite{mixformer}&CVPR22    & 69.2 & 78.7 & 74.7    & -    & -    & -       & 70.7 & 80.0 & 67.8    & -    & -    & 70.4 \\
%     OSTrack-256\cite{ostrack} &ECCV22       & 69.1 & 78.7 & 75.2    & 47.4 & 57.3 & 53.3    & 71.0 & 80.4 & 68.2    & 54.3 & -    & 68.3\\
%     STARK\cite{stark} & ICCV21              & 67.1 & 77.0 & -       & -    &-     & -       & 68.8 & 78.1 & 64.1    & -    & -    &-     \\
%     AutoMatch\cite{AutoMatch}&ICCV21        & 58.3 &-     & 59.9    & -    & -    &-        & 65.2 & 76.6 & 54.3    & 47.2 & 43.5 & - \\
%     TransT \cite{transt}& CVPR21            & 64.9 & 73.8 & 69.0    & -    & -    & -       & 67.1 & 76.8 & 60.9    & 50.7 & 51.7 & 69.1 \\
%     Ocean \cite{Ocean}&  ECCV 20            & 56.0 & 65.1 & 56.6    &-     & -    &-        & 61.1 & 72.1 & 47.3    & 38.4 & 37.7 &-     \\
%     SiamRPN++\cite{SiamRPN++}&CVPR19        & 49.6 & 56.9 & 49.1    & 34.0 & 41.6 & 39.6    & 51.7 & 61.6 & 32.5    & 41.3 & 41.2 & 61.0 \\
%     ECO \cite{ECO} & ICCV 17                & 32.4 & 33.8 & 30.1    & 22.0 & 25.2 & 24.0    & 31.6 & 30.9 & 11.1    & 32.6 & 31.7 & 53.5 \\
%     SiamFC \cite{SiamFC} & ECCVW16          & 33.6 & 42.0 & 33.9    & 23.0 & 31.1 & 26.9    & 34.8 & 35.3 & 9.8     & 29.5 & 28.6 & 46.8 \\
%     \midrule
    
%     \multicolumn{14}{l}{\multirow{1}{*}{\textit{Some Trackers with Higher Resolution}} }\\
%     \midrule
%     OSTrack-384\cite{ostrack}&ECCV22        & 71.1 & 81.1 & 77.6    & 50.5 & 61.3 & 57.6    & 73.7 & 83.2 & 70.8    & 55.9 &-     &70.7  \\
%     % SeqTrack-B384\cite{seqtrack} & CVPR23   & 71.5 & 81.1 & 77.8    & 50.5 & 61.6 & 57.5    & 74.5 & 84.3 & 71.4    & 56.4 & -    & 68.6 \\
%     ARTrack-384\cite{ARTrack} & CVPR23      & 72.6 & 81.7 & 79.1    & 51.9 & 62.0 & 58.5    & 75.5 & 84.3 & 74.3    & 59.8 & -    & 70.5 \\
%     ROMTrack-384\cite{ROMTrack} & ICCV23    & 71.4 & 81.4 & 78.2    & 51.3 & 62.4 & 58.6    & 74.2 & 84.3 & 72.4    & -    & -    & 70.5 \\
%     F-BDMTrack-384\cite{F-BDMTrack}&ICCV23  & 72.0 & 81.5 & 77.7    & 50.8 & 61.3 & 57.8    & 75.4 & 84.3 & 72.9    & 57.8 & 59.4 & 70.9\\
%     ODTrack-B\cite{odtrack} & AAAI24        & 73.2 & 83.2 & 80.6    & 52.4 & 63.9 & 60.1    & 77.0 & 87.9 & 75.1    & 60.9 & -    & -  \\
%     EVPTrack-384\cite{evptrack} & AAAI24    & 72.7 & 82.9 & 80.3    & 53.7 & 65.5 & 61.9    & 76.6 & 86.7 & 73.9    & 59.1 & 62.0 & 70.9  \\
%     ARTrackv2-384\cite{artrackv2} & CVPR24  & 73.0 & 82.0 & 79.6    & 52.9 & 63.4 & 59.1    & 77.5 & 86.0 & 75.5    & 61.6 & -    & 71.7\\
%     AQATrack-384\cite{AQATrack} & CVPR24    & 72.7 & 82.9 & 80.2    & 52.7 & 64.2 & 60.8    & 76.0 & 85.2 & 74.9    & 59.3 & 62.3 & 71.2\\
%     \midrule
%     \textbf{{\mytracker}-384} & Ours        & 73.1 & 83.0 & \bred{80.7}    &&&  &&&  &&&\\
%     \bottomrule    
%     \end{tabular}
%     }
% \caption{ Performance comparisons with state-of-the-art trackers on the test set of LaSOT\cite{lasot}, $\rm LaSOT_{ext}$\cite{lasot-ext} , GOT-10K\cite{got10k}, TNL2K\cite{tnl2k} and UAV123\cite{uav123}. We add a symbol * over GOT-10k to indicate that the corresponding models are only trained with the GOT-10k training set. The top two results are highlighted with \textbf{{\color{red}red}} and \textbf{{\color{blue}blue}} fonts, respectively.}
% \label{tab:1}
% \end{table*} 


\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    % \fontsize{8}{9}\selectfont
    \begin{tabular}{r|c|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{Method} }
    & \multicolumn{1}{c|}{\multirow{2}{*}{Source}} 
    & \multicolumn{3}{c|}{LaSOT} 
    & \multicolumn{3}{c|}{LaSOT$_{ext}$} 
    & \multicolumn{3}{c|}{GOT-10K$^*$} 
    & \multicolumn{3}{c}{TrackingNet}\\
    % & \multicolumn{1}{c}{UAV123}\\ 
    \cline{3-14}
                                            && AUC & P$_{norm}$ & P     & AUC & P$_{norm}$ & P      & AO & SR$_{0.5}$ & SR$_{0.75}$     & AUC & P$_{norm}$ & P \\
    \midrule

    \textbf{{\mytracker}-256} & Ours                 & \bred{72.0} & \bred{82.1} & \bred{79.1}      &\bred{52.4} & \bred{63.3} & \bred{60.2} & \bred{74.9} & \bred{84.8} & 71.7  & \bred{84.3} & \bred{88.8} & \bred{83.5}\\
    \midrule
    AQATrack-256\cite{AQATrack} & CVPR24    & \bblu{71.4} & \bblu{81.9} & \bblu{78.6}    & \bblu{51.2} & \bblu{62.2} & \bblu{58.9}    & 73.8 & 83.2 & \bred{72.1}    & 83.8 & 88.6 & \bblu{83.1}\\
    % ARTrackv2-256\cite{artrackv2} & CVPR24  & \bblu{71.6} & 80.2 & 77.2    & 50.8 & 61.9 & 57.7    & 75.9 & 85.4 & 72.7    &  &  & \\
    EVPTrack-224\cite{evptrack} &AAAI24     & 70.4 & 80.9 & 77.2    & 48.7 & 59.5 & 55.1    & 73.3 & 83.6 & 70.7    & 83.5 & 88.3 & - \\
    F-BDMTrack-256\cite{F-BDMTrack}&ICCV23  & 69.9 & 79.4 & 75.8    & 47.9 & 57.9 & 54.0    & 72.7 & 82.0 & 69.9    & 83.7 & 88.3 & 82.6 \\
    ROMTrack-256\cite{ROMTrack} & ICCV23    & 69.3 & 78.8 & 75.6    & 48.9 & 59.3 & 55.0    & 72.9 & 82.9 & 70.2    & 83.6 & 88.4 & 82.7 \\
    ARTrack-256\cite{ARTrack} & CVPR23      & 70.4 & 79.5 & 76.6    & 46.4 & 56.5 & 52.3    & 73.5 & 82.2 & 70.9    & \bblu{84.2} & \bblu{88.7} & \bred{83.5} \\
    SeqTrack-B256\cite{seqtrack} & CVPR23   & 69.9 & 79.7 & 76.3    & 49.5 & 60.8 & 56.3    & \bblu{74.7} & \bblu{84.7} & \bblu{71.8}    & 83.3 & 88.3    & 82.2 \\
    VideoTrack\cite{VideoTrack1}  & CVPR23  & 70.2 & - & 76.4       & -    & -    & -       & 72.9 & 81.9 & 69.8    & 83.8 & \bblu{88.7} & \bblu{83.1} \\
    MixFormer-22k\cite{mixformer}&CVPR22    & 69.2 & 78.7 & 74.7    & -    & -    & -       & 70.7 & 80.0 & 67.8    & 83.1 & 88.1 & 81.6 \\
    OSTrack-256\cite{ostrack} &ECCV22       & 69.1 & 78.7 & 75.2    & 47.4 & 57.3 & 53.3    & 71.0 & 80.4 & 68.2    & 83.1 & 87.8 & 82.0\\
    STARK-ST101\cite{stark} & ICCV21        & 67.1 & 77.0 & -       & -    &-     & -       & 68.8 & 78.1 & 64.1    & 82.0 & 86.9 & -    \\
    AutoMatch\cite{AutoMatch}&ICCV21        & 58.3 &-     & 59.9    & -    & -    &-        & 65.2 & 76.6 & 54.3    & 76.0 & -    & 72.6 \\
    TransT \cite{transt}& CVPR21            & 64.9 & 73.8 & 69.0    & -    & -    & -       & 67.1 & 76.8 & 60.9    & 81.4 & 86.7 & 80.3 \\
    Ocean \cite{Ocean}&  ECCV 20            & 56.0 & 65.1 & 56.6    &-     & -    &-        & 61.1 & 72.1 & 47.3    & -    & -    &-     \\
    SiamRPN++\cite{SiamRPN++}&CVPR19        & 49.6 & 56.9 & 49.1    & 34.0 & 41.6 & 39.6    & 51.7 & 61.6 & 32.5    & 73.3 & 80.0 & 69.4 \\
    ECO \cite{ECO} & ICCV 17                & 32.4 & 33.8 & 30.1    & 22.0 & 25.2 & 24.0    & 31.6 & 30.9 & 11.1    & -    & -    & - \\
    SiamFC \cite{SiamFC} & ECCVW16          & 33.6 & 42.0 & 33.9    & 23.0 & 31.1 & 26.9    & 34.8 & 35.3 & 9.8     & -    & -    & - \\
    \midrule
    
    \multicolumn{14}{l}{\multirow{1}{*}{\textit{Some Trackers with Higher Resolution}} }\\
    \midrule
    OSTrack-384\cite{ostrack}&ECCV22        & 71.1 & 81.1 & 77.6    & 50.5 & 61.3 & 57.6    & 73.7 & 83.2 & 70.8    & 83.9 & 88.5 & 83.2  \\
    ROMTrack-384\cite{ROMTrack} & ICCV23    & 71.4 & 81.4 & 78.2    & 51.3 & 62.4 & 58.6    & 74.2 & 84.3 & 72.4    & 84.1 & 89.0 & 83.7 \\
    F-BDMTrack-384\cite{F-BDMTrack}&ICCV23  & 72.0 & 81.5 & 77.7    & 50.8 & 61.3 & 57.8    & 75.4 & 84.3 & 72.9    & 84.5 & 89.0 & 84.0\\
    SeqTrack-B384\cite{seqtrack} & CVPR23   & 71.5 & 81.1 & 77.8    & 50.5 & 61.6 & 57.5    & 74.5 & 84.3 & 71.4    & 83.9 & 88.8 & 83.6 \\
    ARTrack-384\cite{ARTrack} & CVPR23      & 72.6 & 81.7 & 79.1    & 51.9 & 62.0 & 58.5    & 75.5 & 84.3 & 74.3    & \bred{85.1} & \bblu{89.1} & \bred{84.8} \\
    % ODTrack-B\cite{odtrack} & AAAI24        & 73.2 & 83.2 & 80.6    & 52.4 & 63.9 & 60.1    & 77.0 & 87.9 & 75.1    & 85.1 & 90.1 & 84.9  \\
    % EVPTrack-384\cite{evptrack} & AAAI24    & \bblu{72.7} & \bblu{82.9} & \bblu{80.3}    & \bred{53.7} & \bred{65.5} & \bred{61.9}    & 76.6 & 86.7 & 73.9    & 84.4 & \bblu{89.1} & -  \\
    % ARTrackv2-384\cite{artrackv2} & CVPR24  & 73.0 & 82.0 & 79.6    & 52.9 & 63.4 & 59.1    & 77.5 & 86.0 & 75.5    & 85.7 & 89.8 & 85.5\\
    HIPTrack\cite{hiptrack}    & CVPR24     & \bblu{72.7} & \bblu{82.9} & 79.5    & \bblu{53.0} & \bblu{64.3} & 60.6    & \bred{77.4} & \bred{88.0} & \bblu{74.5}    & 84.5 & \bblu{89.1} & 83.8\\
    AQATrack-384\cite{AQATrack} & CVPR24    & \bblu{72.7} & \bblu{82.9} & \bblu{80.2}    & 52.7 & 64.2 & \bblu{60.8}    & 76.0 & \bblu{85.2} & \bred{74.9}  & 84.8 & \bred{89.3} & \bblu{84.3}\\
    \midrule
    \textbf{{\mytracker}-384} & Ours        & \bred{73.1} & \bred{83.0} & \bred{80.7}    & \bred{53.4} & \bred{64.8} & \bred{61.0}    & \bblu{76.1} & 84.9 & 74.4 & \bblu{85.0} & \bred{89.3} & \bred{84.8}\\
    \bottomrule    
    \end{tabular}
    }
\caption{ Performance comparisons with state-of-the-art trackers on the test set of LaSOT\cite{lasot}, $\rm LaSOT_{ext}$\cite{lasot-ext} , GOT-10K\cite{got10k} and Trackingnet\cite{trackingnet}. We add a symbol * over GOT-10k to indicate that the corresponding models are only trained with the GOT-10k training set. The top two results are highlighted with \textbf{{\color{red}red}} and \textbf{{\color{blue}blue}} fonts, respectively.}
\label{tab:1}
\end{table*} 


==> tables/tab2.tex <==
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{
%     \fontsize{9}{12}\selectfont
%     \begin{tabular}{c|cccccccccc|cc}
%     \toprule
%                    &SiamFC &ECO  &SiamRPN++ &TransT &MixFormer-22k &OSTrack &ARTrack &F-BDMTrack &EVPTrack &AQATrack &\textbf{Ours-256} & \textbf{Ours-384}\\ 
%     \cline{1-13}
%     AUC            &57.1   &55.4 &73.3      &81.4   &83.1          &83.9    &85.1    &83.7       & 84.4    & 84.8    &  84.3 &  \\ %ep148
%     $\rm P_{Norm}$ &66.3   &61.8 &80.0      &86.7   &88.1          &88.5    &89.1    &88.3       & 89.1    & 89.3    &  88.8 &  \\
%     P              &53.3   &49.2 &69.4      &80.3   &81.6          &83.2    &84.8    &82.6       & -       & 84.3    &  83.5 &  \\
%     \bottomrule 
%     \end{tabular}}

% \caption{ Performance comparisons with state-of-the-art trackers on the test set of TrackingNet\cite{trackingnet}. The top two results are highlighted with \textbf{{\color{red}red}} and \textbf{{\color{blue}blue}} fonts respectively.}

% \label{tab:2}
% \end{table*} 

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    % \fontsize{9}{11}\selectfont
    \begin{tabular}{c|cccccccccc|c}
    \toprule
    %            &SiamFC &ECO   &SiamRPN++ &TransT &OSTrack & SeqTrack &ARTrack &F-BDMTrack &EVPTrack &AQATrack & ODTrack &\textbf{\mytracker-256} & \textbf{\mytracker-384}  \\ 
    % \cline{1-14} %256或者224尺寸的
    % AUC        & 29.5  & 32.6 & 41.3     & 50.7  & 55.9   & 56.4     & 59.8   & 57.8      & 59.1    & 59.3    & 60.9 & 58.8  &                 \\ 
    % P          & 28.6  & 31.7 & 41.2     & 51.7  & -      & -        & 57.5   & 59.4      & 62.0    & 62.3    &   -  & 60.9  &                \\ 


               &SiamFC &ECO   &SiamRPN++   &TransT &OSTrack & SeqTrack &ARTrack &F-BDMTrack &EVPTrack &AQATrack &{\mytracker} \\ 
    \cline{1-12} %256或者224尺寸的
    TNL2K        & 29.5  & 32.6 & 41.3     & 50.7  & 54.3   & 54.9     & 57.5   & 56.4      & 57.5    & \bblu{57.8}        & \bred{58.8}                \\ 
    % P          & 28.6  & 31.7 & 41.2     & 51.7  & -      & -        & -      & 56.5      & 58.8    & 59.4        &                \\ 
    UAV123       & 46.8  & 53.5 & 61.0     & 69.1  & 68.3   & 69.2     & 67.7   & 69.0      & 70.2    & \bblu{70.7} & \bred{70.8}                  \\
    \bottomrule  
    \end{tabular}}

\caption{ Performance comparisons with state-of-the-art trackers on the TNL2K\cite{tnl2k}. The top one results are highlighted with \textbf{{\color{red}red}} fonts respectively.}

\label{tab:2}
\end{table*} 



==> tables/tbl-backbone_num_frames.tex <==
% \begin{table}[t]
%     \centering
%     % \resizebox{\linewidth}{!}{
%         \fontsize{9}{9}\selectfont
%         \begin{tabular}{c|c|ccc}
%         \toprule
%          Encoder & {\mymodule} &AUC & P$_{norm}$ &P\\
%          \midrule
%           & \checkmark & 69.6 & 79.5 & 75.6\\ %141
%          & \checkmark & \textbf{71.4} & \textbf{81.9} & \textbf{78.6} \\
%          & \checkmark & \textbf{71.4} & \textbf{81.9} & \textbf{78.6} \\
%         \bottomrule 
%         \end{tabular}
%         % }
        
%     \caption{ The effectiveness of our method using other backbones on LaSOT\cite{lasot}.}
%     \label{tab:encoder}
% \end{table} 


\begin{table}[t]
    % \centering
    %     % \resizebox{\linewidth}{!}{
    %     \fontsize{9}{9}\selectfont
    %     \begin{tabular}{c|c|ccc}
    %     \toprule
    %      m & n & AUC & P$_{norm}$  & P \\
    %      \midrule
    %      2  & 16 & 71.1 & 81.2 & 78.2\\
    %      4  & 8  & 71.9 & 82.0 & 79.0\\
    %      8  & 4  & 72.0  & 82.1 & 79.1\\
    %      % 16 & 2  &  & & \\
    %     \bottomrule 
    %     \end{tabular}
    %     % }    
    % \caption{ The influence of the size of sliding window.}
    % \label{tab:temporal_number}
    \centering
        % \resizebox{\linewidth}{!}{
        \fontsize{9}{9}\selectfont
        \begin{tabular}{c|cc|cc}
        \toprule 
         \multirow{2}{*}{Method}  &\multicolumn{2}{c|}{LaSOT} &\multicolumn{2}{c}{GOT10K}  \\
         \cline{2-5}
         & AUC & P$_{norm}$ & AO & SR$_{0.5}$ \\
         \midrule
         Baseline  & 71.1  & 81.2 & 73.0 & 82.8 \\
         +{\mytoken} & 71.4 & 81.5 & 73.7 & 83.3 \\ %不进行时序建模，直接指导search
         +{\mymodule} & 72.0 & 82.1 & 74.9 & 84.8  \\
        \bottomrule 
        \end{tabular}
        % }
    \caption{Ablation studies of {\mytracker}.}
    \label{tab:ablation}
\end{table} 


% \begin{table*}[ht]
%     \centering
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         % \resizebox{\linewidth}{!}{
%         \fontsize{10}{9}\selectfont
%         \begin{tabular}{c|ccc}
%         \toprule
%          Backbone &  AUC & P$_{norm}$ & P\\
%          \midrule
%          ViT            &  &  & \\
%          HiViT          &  &  & \\ %不进行时序建模，直接指导search
%          \textbf{iTPN}  & \textbf{72.5} & \textbf{82.9} & \textbf{80.1} \\
%         \bottomrule 
%         \end{tabular}
%         %} 
%     \subcaption{Compare different number of {\mymodule}.}
%     \label{tab:temporal_number}
%     \end{minipage}
%     % \hfill
%     \hspace{0.01\textwidth} % Space between the tables
%     \begin{minipage}{0.43\linewidth}
%         \centering
%         \resizebox{\linewidth}{!}{
%         \fontsize{9}{9}\selectfont
%         \begin{tabular}{c|c|cc}
%         \toprule
%          m & n & AUC & P$_{norm}$  \\%& P \\
%          \midrule
%          2  & 16 &  & \\%& 77.5 \\
%          \textbf{4}  & \textbf{8}  &  & \\ %\textbf{78.6} \\
%          8  & 4  &  & \\%& 77.7  \\
%          16 & 2  &  & \\%& 77.3  \\
%         \bottomrule 
%         \end{tabular}
%         }
%     \subcaption{Compare different sequence lengths.}
%     \label{tab:temporal_length}
%     \end{minipage}
%     \caption{The effective from different numbers of {\mymodule} and sequence length.}
%     \label{tab: numder}
    
% \end{table*}

==> tables/tbl-fps.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
        \fontsize{9}{11}\selectfont
        \begin{tabular}{c|ccccc}
        \toprule
         Model & Params(M)& FLOPs(G)  & Speed(FPS)  \\
         \midrule
         % SeqTrack-256\cite{seqtrack} & 2080Ti & 89 & 66   & 40  \\
         % STARK\cite{stark}& Tesla v100 & 43.4 & 18.5  & 31.7   \\
         % \midrule
         % ARTrack-256\cite{ARTrack} & 173 & 37  & 27   \\
         % ARTrack-384\cite{ARTrack} & 173 & 83  & 20   \\
         SeqTrack-B256\cite{seqtrack} & 89 & 65  & 40  \\
         SeqTrack-B384\cite{seqtrack} & 89 & 148  & 15 \\ 
         % ODTrack-B\cite{ostrack} & 92  & 73  & 47 \\
         {\mytracker}-256(ours)   & 70  & 24.8 & 46 \\
         {\mytracker}-384(ours)   & 70  & 55.7 & 36 \\
        \bottomrule 
        \end{tabular}
    }
    
    \caption{ Comparison of model Params, FLOPs, and Speed on NVIDIA V100.}
    \label{tab:fps}
\end{table} 
